iMARS: An In-Memory-Computing Architecture for Recommendation Systems

Recommendation systems (RecSys) suggest items to users by predicting their preferences based on historical data. Typical RecSys handle large embedding tables and many embedding table related operations. The memory size and bandwidth of the conventional computer architecture restrict the performance of RecSys. This work proposes an in-memory-computing (IMC) architecture (iMARS) for accelerating the filtering and ranking stages of deep neural network-based RecSys. iMARS leverages IMC-friendly embedding tables implemented inside a ferroelectric FET based IMC fabric. Circuit-level and system-level evaluation show that \fw achieves 16.8x (713x) end-to-end latency (energy) improvement compared to the GPU counterpart for the MovieLens dataset.

==> Figures/end2end_eval.tex <==
\pgfplotstableread[row sep=\\,col sep=&]{
HW &	Embedding	&	ANN	&	KNN		\\
GPU	 &	10	&	40	&	50	\\
IBET &	20	&	50	&	30	\\
CBET &	30	&	60	&	10	\\
    }\enddelay
    
\pgfplotstableread[row sep=\\,col sep=&]{
HW &	Embedding	&	ANN	&	KNN		\\
GPU	 &	10	&	40	&	50	\\
IBET &	20	&	50	&	30	\\
CBET &	30	&	60	&	10	\\
    }\endenergy

 
\begin{figure}
    \centering
    \sansmath\sffamily
    \hspace{-1.5cm}
    \begin{subfigure}[t]{0.2\textwidth}
    \raggedleft
    \begin{tikzpicture}
        \begin{axis}[
            width=1.0*\textwidth,
            height=1.0*\textwidth,
            bar width = 0.1*\textwidth,
            enlarge x limits = 0.3,
            legend style={fill=white,draw=white},
            legend columns=1,
            legend pos = outer north east,
            legend cell align = left,
            reverse legend,
        	ybar stacked,
            %xlabel={Latency},
            ylabel style={align=center}, 
            ylabel={(a) Execution Time (s)},
            xtick={GPU, IBET, CBET},
            symbolic x coords={GPU, IBET, CBET},
            xticklabels={GPU, IBET, CBET},
            ymin=0,
            ymax=100,
            %tick label style={font=\footnotesize},
            ]
            \addplot [color=black, fill=modern_yellow] table[x=HW,y=Embedding]{\enddelay};
            \addplot [color=black, fill=modern_green] table[x=HW,y=ANN]{\enddelay};
            \addplot [color=black, fill=modern_blue] table[x=HW,y=KNN]{\enddelay};
            
        %\legend{Embedding, ANN, KNN}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure} \hspace{0.1cm}
    \begin{subfigure}[t]{0.2\textwidth}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            width=1.0*\textwidth,
            height=1.0*\textwidth,
            bar width = 0.1*\textwidth,
            enlarge x limits = 0.3,
            legend style={fill=white,draw=white},
            legend columns=1,
            legend pos = outer north east,
            legend cell align = left,
            reverse legend,
        	ybar stacked,
            %xlabel={Energy},
            ylabel style={align=center}, 
            ylabel={(b) Energy (fJ)},
            xtick={GPU, IBET, CBET},
            symbolic x coords={GPU, IBET, CBET},
            xticklabels={GPU, IBET, CBET},
            ymin=0,
            ymax=100,
            %tick label style={font=\footnotesize},
            ]
            \addplot [color=black, fill=modern_yellow] table[x=HW,y=Embedding]{\endenergy};
            \addplot [color=black, fill=modern_green] table[x=HW,y=ANN]{\endenergy};
            \addplot [color=black, fill=modern_blue] table[x=HW,y=KNN]{\endenergy};
            
        \legend{Embedding, ANN, KNN}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure}
    \caption{End-to-End Latency and Energy \Note{Wrong values need to update}}
    \label{fig:end2end_eval}
\end{figure}

==> Figures/et_eval.tex <==
\pgfplotstableread[row sep=\\,col sep=&]{
HW &	Embedding	&	ANN	&	KNN		\\
GPU	 &	10	&	40	&	50	\\
IBET &	20	&	50	&	30	\\
    }\iecgdelay
    
\pgfplotstableread[row sep=\\,col sep=&]{
HW &	Embedding	&	ANN	&	KNN		\\
GPU	 &	10	&	40	&	50	\\
IBET &	20	&	50	&	30	\\
    }\iecgenergy
    
\pgfplotstableread[row sep=\\,col sep=&]{
HW &	Embedding	&	ANN	&	KNN		\\
GPU	 &	10	&	40	&	50	\\
IBET &	20	&	50	&	30	\\
    }\ierdelay
    
\pgfplotstableread[row sep=\\,col sep=&]{
HW &	Embedding	&	ANN	&	KNN		\\
GPU	 &	10	&	40	&	50	\\
IBET &	20	&	50	&	30	\\
    }\ierenergy
    
\pgfplotstableread[row sep=\\,col sep=&]{
HW &	Embedding	&	ANN	&	KNN		\\
GPU	 &	10	&	40	&	50	\\
IBET &	20	&	50	&	30	\\
    }\ieenddelay
    
\pgfplotstableread[row sep=\\,col sep=&]{
HW &	Embedding	&	ANN	&	KNN		\\
GPU	 &	10	&	40	&	50	\\
IBET &	20	&	50	&	30	\\
    }\ieendenergy

 
\begin{figure}
    \centering
    \sansmath\sffamily
    
    \textbf{Candidate Generation} \\
    \hspace{-1.5cm}
    \begin{subfigure}[t]{0.2\textwidth}
    \raggedleft
    \begin{tikzpicture}
        \begin{axis}[
            width=1.0*\textwidth,
            height=1.0*\textwidth,
            bar width = 0.1*\textwidth,
            enlarge x limits = 0.3,
            legend style={fill=white,draw=white},
            legend columns=1,
            legend pos = outer north east,
            legend cell align = left,
            reverse legend,
        	ybar stacked,
            %xlabel={Latency},
            ylabel style={align=center}, 
            ylabel={(a) Execution Time (s)},
            xtick={GPU, IBET, CBET},
            symbolic x coords={GPU, IBET, CBET},
            xticklabels={GPU, IBET},
            ymin=0,
            ymax=100,
            %tick label style={font=\footnotesize},
            ]
            \addplot [color=black, fill=modern_yellow] table[x=HW,y=Embedding]{\iecgdelay};
            \addplot [color=black, fill=modern_green] table[x=HW,y=ANN]{\iecgdelay};
            \addplot [color=black, fill=modern_blue] table[x=HW,y=KNN]{\iecgdelay};
            
        %\legend{Embedding, ANN, KNN}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure} \hspace{0.1cm}
    \begin{subfigure}[t]{0.2\textwidth}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            width=1.0*\textwidth,
            height=1.0*\textwidth,
            bar width = 0.1*\textwidth,
            enlarge x limits = 0.3,
            legend style={fill=white,draw=white},
            legend columns=1,
            legend pos = outer north east,
            legend cell align = left,
            reverse legend,
        	ybar stacked,
            %xlabel={Energy},
            ylabel style={align=center}, 
            ylabel={(b) Energy (fJ)},
            xtick={GPU, IBET, CBET},
            symbolic x coords={GPU, IBET, CBET},
            xticklabels={GPU, IBET, CBET},
            ymin=0,
            ymax=100,
            %tick label style={font=\footnotesize},
            ]
            \addplot [color=black, fill=modern_yellow] table[x=HW,y=Embedding]{\iecgenergy};
            \addplot [color=black, fill=modern_green] table[x=HW,y=ANN]{\iecgenergy};
            \addplot [color=black, fill=modern_blue] table[x=HW,y=KNN]{\iecgenergy};
            
        \legend{Embedding, ANN, KNN}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure}  
    
    \textbf{Ranking} \\
    \hspace{-1.5cm}
    \begin{subfigure}[t]{0.2\textwidth}
    \raggedleft
    \begin{tikzpicture}
        \begin{axis}[
            width=1.0*\textwidth,
            height=1.0*\textwidth,
            bar width = 0.1*\textwidth,
            enlarge x limits = 0.3,
            legend style={fill=white,draw=white},
            legend columns=1,
            legend pos = outer north east,
            legend cell align = left,
            reverse legend,
        	ybar stacked,
            %xlabel={Latency},
            ylabel style={align=center}, 
            ylabel={(c) Execution Time (s)},
            xtick={GPU, IBET, CBET},
            symbolic x coords={GPU, IBET, CBET},
            xticklabels={GPU, IBET},
            ymin=0,
            ymax=100,
            %tick label style={font=\footnotesize},
            ]
            \addplot [color=black, fill=modern_yellow] table[x=HW,y=Embedding]{\ierdelay};
            \addplot [color=black, fill=modern_green] table[x=HW,y=ANN]{\ierdelay};
            \addplot [color=black, fill=modern_blue] table[x=HW,y=KNN]{\ierdelay};
            
        %\legend{Embedding, ANN, KNN}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure} \hspace{0.1cm}
    \begin{subfigure}[t]{0.2\textwidth}
    \raggedleft
    \begin{tikzpicture}
        \begin{axis}[
            width=1.0*\textwidth,
            height=1.0*\textwidth,
            bar width = 0.1*\textwidth,
            enlarge x limits = 0.3,
            legend style={fill=white,draw=white},
            legend columns=1,
            legend pos = outer north east,
            legend cell align = left,
            reverse legend,
        	ybar stacked,
            %xlabel={Latency},
            ylabel style={align=center}, 
            ylabel={(d) Energy (fJ)},
            xtick={GPU, IBET, CBET},
            symbolic x coords={GPU, IBET, CBET},
            xticklabels={GPU, IBET},
            ymin=0,
            ymax=100,
            %tick label style={font=\footnotesize},
            ]
            \addplot [color=black, fill=modern_yellow] table[x=HW,y=Embedding]{\ierenergy};
            \addplot [color=black, fill=modern_green] table[x=HW,y=ANN]{\ierenergy};
            \addplot [color=black, fill=modern_blue] table[x=HW,y=KNN]{\ierenergy};
            
        \legend{Embedding, ANN, TopK}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure} 
    
    \textbf{End-to-End} \\
    \hspace{-1.5cm}
    \begin{subfigure}[t]{0.2\textwidth}
    \raggedleft
    \begin{tikzpicture}
        \begin{axis}[
            width=1.0*\textwidth,
            height=1.0*\textwidth,
            bar width = 0.1*\textwidth,
            enlarge x limits = 0.3,
            legend style={fill=white,draw=white},
            legend columns=1,
            legend pos = outer north east,
            legend cell align = left,
            reverse legend,
        	ybar stacked,
            %xlabel={Latency},
            ylabel style={align=center}, 
            ylabel={(e) Execution Time (s)},
            xtick={GPU, IBET, CBET},
            symbolic x coords={GPU, IBET, CBET},
            xticklabels={GPU, IBET},
            ymin=0,
            ymax=100,
            %tick label style={font=\footnotesize},
            ]
            \addplot [color=black, fill=modern_yellow] table[x=HW,y=Embedding]{\ieenddelay};
            \addplot [color=black, fill=modern_green] table[x=HW,y=ANN]{\ieenddelay};
            \addplot [color=black, fill=modern_blue] table[x=HW,y=KNN]{\ieenddelay};
            
        %\legend{Embedding, ANN, KNN}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure} \hspace{0.1cm}
    \begin{subfigure}[t]{0.2\textwidth}
    \raggedleft
    \begin{tikzpicture}
        \begin{axis}[
            width=1.0*\textwidth,
            height=1.0*\textwidth,
            bar width = 0.1*\textwidth,
            enlarge x limits = 0.3,
            legend style={fill=white,draw=white},
            legend columns=1,
            legend pos = outer north east,
            legend cell align = left,
            reverse legend,
        	ybar stacked,
            %xlabel={Latency},
            ylabel style={align=center}, 
            ylabel={(f) Energy (fJ)},
            xtick={GPU, IBET, CBET},
            symbolic x coords={GPU, IBET, CBET},
            xticklabels={GPU, IBET},
            ymin=0,
            ymax=100,
            %tick label style={font=\footnotesize},
            ]
            \addplot [color=black, fill=modern_yellow] table[x=HW,y=Embedding]{\ieendenergy};
            \addplot [color=black, fill=modern_green] table[x=HW,y=ANN]{\ieendenergy};
            \addplot [color=black, fill=modern_blue] table[x=HW,y=KNN]{\ieendenergy};
            
        \legend{Embedding, ANN, KNN}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure} \hspace{0.1cm}
    \caption{Latency and Energy for Ranking \Note{Wrong values need to update}}
    \label{fig:category_eva}
\end{figure}

==> Figures/itembased_eval.tex <==
\pgfplotstableread[row sep=\\,col sep=&]{
HW &	Embedding	&	ANN	        & KNN	   \\
GPU	 &	4.97E-06	&   1.26E-05	& 1.59E-05 \\
IBET &  2.50E-10	&   1.13E-06	& 1.81E-10 \\
    }\iecgdelay
    
\pgfplotstableread[row sep=\\,col sep=&]{
HW &	Embedding	&	ANN	&	KNN		\\
GPU	 &	10	&	40	&	50	\\
IBET &	20	&	50	&	30	\\
    }\iecgenergy
    
\pgfplotstableread[row sep=\\,col sep=&]{
HW &	Embedding	&	ANN	&	KNN		\\
GPU	 &	10	&	40	&	50	\\
IBET &	20	&	50	&	30	\\
    }\ierdelay
    
\pgfplotstableread[row sep=\\,col sep=&]{
HW &	Embedding	&	ANN	&	KNN		\\
GPU	 &	10	&	40	&	50	\\
IBET &	20	&	50	&	30	\\
    }\ierenergy
    
\pgfplotstableread[row sep=\\,col sep=&]{
HW &	Embedding	&	ANN	&	KNN		\\
GPU	 &	10	&	40	&	50	\\
IBET &	20	&	50	&	30	\\
    }\ieenddelay
    
\pgfplotstableread[row sep=\\,col sep=&]{
HW &	Embedding	&	ANN	&	KNN		\\
GPU	 &	10	&	40	&	50	\\
IBET &	20	&	50	&	30	\\
    }\ieendenergy

 
\begin{figure}
    \centering
    \sansmath\sffamily
    
    \textbf{Candidate Generation} \\
    \hspace{-1.5cm}
    \begin{subfigure}[t]{0.2\textwidth}
    \raggedleft
    \begin{tikzpicture}
        \begin{axis}[
            width=1.0*\textwidth,
            height=1.0*\textwidth,
            bar width = 0.1*\textwidth,
            enlarge x limits = 0.3,
            legend style={fill=white,draw=white},
            legend columns=1,
            legend pos = outer north east,
            legend cell align = left,
            reverse legend,
        	ybar stacked,
            %xlabel={Latency},
            ylabel style={align=center}, 
            ylabel={(a) Execution Time (s)},
            xtick={GPU, IBET},
            symbolic x coords={GPU, IBET},
            xticklabels={GPU, IBET},
            %ymin=0,
            %ymax=100,
            %tick label style={font=\footnotesize},
            ]
            \addplot [color=black, fill=modern_yellow] table[x=HW,y=Embedding]{\iecgdelay};
            \addplot [color=black, fill=modern_green] table[x=HW,y=ANN]{\iecgdelay};
            \addplot [color=black, fill=modern_blue] table[x=HW,y=KNN]{\iecgdelay};
            
        %\legend{Embedding, ANN, KNN}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure} \hspace{0.1cm}
    \begin{subfigure}[t]{0.2\textwidth}
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            width=1.0*\textwidth,
            height=1.0*\textwidth,
            bar width = 0.1*\textwidth,
            enlarge x limits = 0.3,
            legend style={fill=white,draw=white},
            legend columns=1,
            legend pos = outer north east,
            legend cell align = left,
            reverse legend,
        	ybar stacked,
            %xlabel={Energy},
            ylabel style={align=center}, 
            ylabel={(b) Energy (fJ)},
            xtick={GPU, IBET, CBET},
            symbolic x coords={GPU, IBET, CBET},
            xticklabels={GPU, IBET, CBET},
            ymin=0,
            ymax=100,
            %tick label style={font=\footnotesize},
            ]
            \addplot [color=black, fill=modern_yellow] table[x=HW,y=Embedding]{\iecgenergy};
            \addplot [color=black, fill=modern_green] table[x=HW,y=ANN]{\iecgenergy};
            \addplot [color=black, fill=modern_blue] table[x=HW,y=KNN]{\iecgenergy};
            
        \legend{Embedding, ANN, KNN}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure}  
    
    \textbf{Ranking} \\
    \hspace{-1.5cm}
    \begin{subfigure}[t]{0.2\textwidth}
    \raggedleft
    \begin{tikzpicture}
        \begin{axis}[
            width=1.0*\textwidth,
            height=1.0*\textwidth,
            bar width = 0.1*\textwidth,
            enlarge x limits = 0.3,
            legend style={fill=white,draw=white},
            legend columns=1,
            legend pos = outer north east,
            legend cell align = left,
            reverse legend,
        	ybar stacked,
            %xlabel={Latency},
            ylabel style={align=center}, 
            ylabel={(c) Execution Time (s)},
            xtick={GPU, IBET, CBET},
            symbolic x coords={GPU, IBET, CBET},
            xticklabels={GPU, IBET},
            ymin=0,
            ymax=100,
            %tick label style={font=\footnotesize},
            ]
            \addplot [color=black, fill=modern_yellow] table[x=HW,y=Embedding]{\ierdelay};
            \addplot [color=black, fill=modern_green] table[x=HW,y=ANN]{\ierdelay};
            \addplot [color=black, fill=modern_blue] table[x=HW,y=KNN]{\ierdelay};
            
        %\legend{Embedding, ANN, KNN}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure} \hspace{0.1cm}
    \begin{subfigure}[t]{0.2\textwidth}
    \raggedleft
    \begin{tikzpicture}
        \begin{axis}[
            width=1.0*\textwidth,
            height=1.0*\textwidth,
            bar width = 0.1*\textwidth,
            enlarge x limits = 0.3,
            legend style={fill=white,draw=white},
            legend columns=1,
            legend pos = outer north east,
            legend cell align = left,
            reverse legend,
        	ybar stacked,
            %xlabel={Latency},
            ylabel style={align=center}, 
            ylabel={(d) Energy (fJ)},
            xtick={GPU, IBET, CBET},
            symbolic x coords={GPU, IBET, CBET},
            xticklabels={GPU, IBET},
            ymin=0,
            ymax=100,
            %tick label style={font=\footnotesize},
            ]
            \addplot [color=black, fill=modern_yellow] table[x=HW,y=Embedding]{\ierenergy};
            \addplot [color=black, fill=modern_green] table[x=HW,y=ANN]{\ierenergy};
            \addplot [color=black, fill=modern_blue] table[x=HW,y=KNN]{\ierenergy};
            
        \legend{Embedding, ANN, TopK}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure} 
    
    \textbf{End-to-End} \\
    \hspace{-1.5cm}
    \begin{subfigure}[t]{0.2\textwidth}
    \raggedleft
    \begin{tikzpicture}
        \begin{axis}[
            width=1.0*\textwidth,
            height=1.0*\textwidth,
            bar width = 0.1*\textwidth,
            enlarge x limits = 0.3,
            legend style={fill=white,draw=white},
            legend columns=1,
            legend pos = outer north east,
            legend cell align = left,
            reverse legend,
        	ybar stacked,
            %xlabel={Latency},
            ylabel style={align=center}, 
            ylabel={(e) Execution Time (s)},
            xtick={GPU, IBET, CBET},
            symbolic x coords={GPU, IBET, CBET},
            xticklabels={GPU, IBET},
            ymin=0,
            ymax=100,
            %tick label style={font=\footnotesize},
            ]
            \addplot [color=black, fill=modern_yellow] table[x=HW,y=Embedding]{\ieenddelay};
            \addplot [color=black, fill=modern_green] table[x=HW,y=ANN]{\ieenddelay};
            \addplot [color=black, fill=modern_blue] table[x=HW,y=KNN]{\ieenddelay};
            
        %\legend{Embedding, ANN, KNN}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure} \hspace{0.1cm}
    \begin{subfigure}[t]{0.2\textwidth}
    \raggedleft
    \begin{tikzpicture}
        \begin{axis}[
            width=1.0*\textwidth,
            height=1.0*\textwidth,
            bar width = 0.1*\textwidth,
            enlarge x limits = 0.3,
            legend style={fill=white,draw=white},
            legend columns=1,
            legend pos = outer north east,
            legend cell align = left,
            reverse legend,
        	ybar stacked,
            %xlabel={Latency},
            ylabel style={align=center}, 
            ylabel={(f) Energy (fJ)},
            xtick={GPU, IBET, CBET},
            symbolic x coords={GPU, IBET, CBET},
            xticklabels={GPU, IBET},
            ymin=0,
            ymax=100,
            %tick label style={font=\footnotesize},
            ]
            \addplot [color=black, fill=modern_yellow] table[x=HW,y=Embedding]{\ieendenergy};
            \addplot [color=black, fill=modern_green] table[x=HW,y=ANN]{\ieendenergy};
            \addplot [color=black, fill=modern_blue] table[x=HW,y=KNN]{\ieendenergy};
            
        \legend{Embedding, ANN, KNN}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure} \hspace{0.1cm}
    \caption{Latency and Energy for Ranking \Note{Wrong values need to update}}
    \label{fig:item_eva}
\end{figure}

==> Figures/results.tex <==
\pgfplotstableread[row sep=\\,col sep=&]{
HW &	GPU	&	imars\\
Emb	 &	51224	&	83\\
DNN &	15550	&	6228\\
KNN &	75006	&	1\\
    }\filteringlatency
    
\pgfplotstableread[row sep=\\,col sep=&]{
HW &	GPU	&	imars\\
Emb	 &	6e6	&	1e2\\
DNN &	2e6	&	1e0\\
KNN &	8e6	&	2e2\\
    }\filteringenergy
    
\pgfplotstableread[row sep=\\,col sep=&]{
HW &	GPU	&	imars\\
Emb	 &	642	&	1\\
DNN &	122	&	75\\
%KNN &	87812	&	1\\
    }\movielenslatency
    
\pgfplotstableread[row sep=\\,col sep=&]{
HW &	GPU	&	imars\\
Emb	 &	6e6	&	8\\
DNN &	1e6	&	1e0\\
%KNN &	87812	&	1\\
    }\movielensenergy
    
\pgfplotstableread[row sep=\\,col sep=&]{
HW &	GPU	&	imars\\
Emb	 &	155	&	1\\
DNN &	33	&	8\\
%KNN &	87812	&	1\\
    }\kagglelatency
    
\pgfplotstableread[row sep=\\,col sep=&]{
HW &	GPU	&	imars\\
Emb	 &	2e7	&	1e4\\
DNN &	5e6	&	1e0\\
%KNN &	87812	&	1\\
    }\kaggleenergy

 
\begin{figure}
    \centering
    \sansmath\sffamily
    \centering
    %\textbf{Candidate Generation} \\
    \begin{subfigure}[t]{0.15\textwidth}
        \centering
        \begin{tikzpicture} 
            \begin{axis}[%
            legend style={fill=white,draw=white,column sep=0.1cm},
                    legend columns=3,
                    legend cell align = left,
                    legend pos = north east,,
            hide axis,
            width=\textwidth,
            height=\textwidth,
            xmin=10,
            xmax=50,
            ymin=0,
            ymax=0.4,
            ybar stacked,
            ]
            \addlegendimage{color=black,fill=modern_blue}
            \addlegendentry{GPU  };
            \addlegendimage{color=white,fill=white}
            \addlegendentry{  };
            \hspace{0.5cm}
            \addlegendimage{color=black,fill=modern_green}
            \addlegendentry{\fw};
            
            \end{axis}
        \end{tikzpicture}
        %\caption{Energy, Delay and EDP Improvements}
    \end{subfigure} 
    
    \begin{subfigure}[t]{0.2\textwidth}
    \raggedleft
    \begin{tikzpicture}
        \begin{axis}[
            width=1.0*\textwidth,
            height=1.0*\textwidth,
            bar width = 0.05*\textwidth,
            enlarge x limits = 0.3,
            legend style={fill=white,draw=white},
            legend columns=1,
            legend pos = outer north east,
            legend cell align = left,
            reverse legend,
        	ybar,
            %xlabel={Latency},
            ylabel style={align=center}, 
            ylabel={(a) Normalized Latency},
            xtick={Emb, DNN, KNN},
            symbolic x coords={Emb, DNN, KNN},
            xticklabels={Emb, DNN, KNN},
            %%ymin=0,
            %ymax=1000000,
            ymode=log,
            %tick label style={font=\footnotesize},
            ]
            \addplot [color=black, fill=modern_blue] table[x=HW,y=GPU]{\filteringlatency};
            \addplot [color=black, fill=modern_green] table[x=HW,y=imars]{\filteringlatency};
            %\addplot [color=black, fill=modern_blue] table[x=HW,y=KNN]{\iecgdelay};
            
        %\legend{Embedding, ANN, KNN}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure}
    \begin{subfigure}[t]{0.2\textwidth}
    \raggedleft
    \begin{tikzpicture}
        \begin{axis}[
            width=1.0*\textwidth,
            height=1.0*\textwidth,
            bar width = 0.05*\textwidth,
            enlarge x limits = 0.3,
            legend style={fill=white,draw=white},
            legend columns=1,
            legend pos = outer north east,
            legend cell align = left,
            reverse legend,
        	ybar,
            %xlabel={Energy},
            ylabel style={align=center}, 
            ylabel={(b) Normalized Energy},
            xtick={Emb, DNN, KNN},
            symbolic x coords={Emb, DNN, KNN},
            xticklabels={Emb, DNN, KNN},
            %%ymin=0,
            %ymax=1000000,
            ymode=log,
            %tick label style={font=\footnotesize},
            ]
            \addplot [color=black, fill=modern_blue] table[x=HW,y=GPU]{\filteringenergy};
            \addplot [color=black, fill=modern_green] table[x=HW,y=imars]{\filteringenergy};
            %\addplot [color=black, fill=modern_blue] table[x=HW,y=KNN]{\iecgdelay};
            
        %\legend{Embedding, ANN, KNN}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure}  
    %\textbf{Ranking} \\
    \begin{subfigure}[t]{0.2\textwidth}
    \raggedleft
    \begin{tikzpicture}
        \begin{axis}[
            width=1.0*\textwidth,
            height=1.0*\textwidth,
            bar width = 0.05*\textwidth,
            enlarge x limits = 0.3,
            legend style={fill=white,draw=white},
            legend columns=1,
            legend pos = outer north east,
            legend cell align = left,
            reverse legend,
        	ybar,
        	ymode=log,
            %xlabel={Latency},
            ylabel style={align=center}, 
            ylabel={(c) Normalized Latency},
            xtick={Emb, DNN, KNN},
            symbolic x coords={Emb, DNN, KNN},
            xticklabels={Emb, DNN, KNN},
            %%ymin=0,
            %ymax=1000000,
            %tick label style={font=\footnotesize},
            ]
            \addplot [color=black, fill=modern_blue] table[x=HW,y=GPU]{\movielenslatency};
            \addplot [color=black, fill=modern_green] table[x=HW,y=imars]{\movielenslatency};
            %\addplot [color=black, fill=modern_blue] table[x=HW,y=KNN]{\iecgdelay};
            
        %\legend{Embedding, ANN, KNN}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure}
    \begin{subfigure}[t]{0.2\textwidth}
    \raggedleft
    \begin{tikzpicture}
        \begin{axis}[
            width=1.0*\textwidth,
            height=1.0*\textwidth,
            bar width = 0.05*\textwidth,
            enlarge x limits = 0.3,
            legend style={fill=white,draw=white},
            legend columns=1,
            legend pos = outer north east,
            legend cell align = left,
            reverse legend,
        	ybar,
        	ymode=log,
            %xlabel={Latency},
            ylabel style={align=center}, 
            ylabel={(d) Normalized Energy},
            xtick={Emb, DNN, KNN},
            symbolic x coords={Emb, DNN, KNN},
            xticklabels={Emb, DNN, KNN},
            %%ymin=0,
            %%ymax=1000000,
            %tick label style={font=\footnotesize},
            ]
            \addplot [color=black, fill=modern_blue] table[x=HW,y=GPU]{\movielensenergy};
            \addplot [color=black, fill=modern_green] table[x=HW,y=imars]{\movielensenergy};
            %\addplot [color=black, fill=modern_blue] table[x=HW,y=KNN]{\iecgdelay};
            
        %\legend{Embedding, ANN, TopK}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure} 
    %\textbf{End-to-End} \\
    \begin{subfigure}[t]{0.2\textwidth}
    \raggedleft
    \begin{tikzpicture}
        \begin{axis}[
            width=1.0*\textwidth,
            height=1.0*\textwidth,
            bar width = 0.05*\textwidth,
            enlarge x limits = 0.3,
            legend style={fill=white,draw=white},
            legend columns=1,
            legend pos = outer north east,
            legend cell align = left,
            reverse legend,
        	ybar,
        	ymode=log,
            %xlabel={Latency},
            ylabel style={align=center}, 
            ylabel={(e) Normalized Latency},
            xtick={Emb, DNN, KNN},
            symbolic x coords={Emb, DNN, KNN},
            xticklabels={Emb, DNN, KNN},
            %ymin=0,
            %%ymax=100,
            %tick label style={font=\footnotesize},
            ]
            \addplot [color=black, fill=modern_blue] table[x=HW,y=GPU]{\kagglelatency};
            \addplot [color=black, fill=modern_green] table[x=HW,y=imars]{\kagglelatency};
            %\addplot [color=black, fill=modern_blue] table[x=HW,y=KNN]{\iecgdelay};
            
        %\legend{Embedding, ANN, KNN}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure} 
    \begin{subfigure}[t]{0.2\textwidth}
    \raggedleft
    \begin{tikzpicture}
        \begin{axis}[
            width=1.0*\textwidth,
            height=1.0*\textwidth,
            bar width = 0.05*\textwidth,
            enlarge x limits = 0.3,
            legend style={fill=white,draw=white},
            legend columns=1,
            legend pos = outer north east,
            legend cell align = left,
            reverse legend,
        	ybar,
        	ymode=log,
            %xlabel={Latency},
            ylabel style={align=center}, 
            ylabel={(f) Normalized Energy},
            xtick={Emb, DNN, KNN},
            symbolic x coords={Emb, DNN, KNN},
            xticklabels={Emb, DNN, KNN},
            %ymin=0,
            %ymax=100,
            %tick label style={font=\footnotesize},
            ]
            \addplot [color=black, fill=modern_blue] table[x=HW,y=GPU]{\kaggleenergy};
            \addplot [color=black, fill=modern_green] table[x=HW,y=imars]{\kaggleenergy};
            %\addplot [color=black, fill=modern_blue] table[x=HW,y=KNN]{\iecgdelay};
            
        %\legend{Embedding, ANN, KNN}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure}
    
I    \caption{The latency and energy comparison of the GPU and \fw for (a-b) the filtering phase and the ranking phase of (c-d) Movielens and (e-f) Kaggle dataset. \notes{consider use table. Need more work here. }}
    \label{fig:eval}
\end{figure}
